OceanBench: The Sea Surface Height Edition

The ocean profoundly influences human activities and plays a critical role in climate regulation. Our understanding has improved over the last decades with the advent of satellite remote sensing data, allowing us to capture essential quantities over the globe, e.g., sea surface height (SSH). However, ocean satellite data presents challenges for information extraction due to their sparsity and irregular sampling, signal complexity, and noise. Machine learning (ML) techniques have demonstrated their capabilities in dealing with large-scale, complex signals. Therefore we see an opportunity for ML models to harness the information contained in ocean satellite data. However, data representation and relevant evaluation metrics can be the defining factors when determining the success of applied ML. The processing steps from the raw observation data to a ML-ready state and from model outputs to interpretable quantities require domain expertise, which can be a significant barrier to entry for ML researchers. OceanBench is a unifying framework that provides standardized processing steps that comply with domain-expert standards. It provides plug-and-play data and pre-configured pipelines for ML researchers to benchmark their models and a transparent configurable framework for researchers to customize and extend the pipeline for their tasks. In this work, we demonstrate the OceanBench framework through a first edition dedicated to SSH interpolation challenges. We provide datasets and ML-ready benchmarking pipelines for the long-standing problem of interpolating observations from simulated ocean satellite data, multi-modal and multi-sensor fusion issues, and transfer-learning to real ocean satellite observations. The OceanBench framework is available at github.com/jejjohnson/oceanbench and the dataset registry is available at github.com/quentinf00/oceanbench-data-registry.

==> content/0_abstract.tex <==
% \begin{abstract}
% The ocean is a key component of the climate system, profoundly influencing human activities. Consequently, a central question for oceanographers revolves around its observation and prediction at different timescales. Similar to various research fields, oceanography has recently witnessed the emergence of machine learning-based methods as an alternative to more domain-specific approaches. But, surprisingly, the adoption of machine learning methods in this field has been arguably slower compared to others. This can be attributed to the complexity of pre-processing tasks in the domain of geospatial data and to the specialized nature of evaluation metrics relevant to ocean science problems. In this context, we introduce \texttt{OceanBench}, a framework designed to lower the barrier to entry for ML researchers by standardizing and automating this process that comply with domain-expert standards.
% It seeks to maintains readability, robustness, and flexibility by providing a standardized framework to explicitly highlight the preprocessing step used, the parameters chosen and the sequence of operations performed. 
% It takes a step towards incorporate these domain-driven decisions to integrate well with existing ML pipelines.
% We demonstrate the usefulness of \texttt{OceanBench} on a series of SSH interpolation tasks with consistent dataflow pipelines, physically-inspired metrics, and interpretable visualizations.

% \end{abstract}

  % The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
  % both the left- and right-hand margins. Use 10~point type, with a vertical
  % spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
  % bold, and in point size 12. Two line spaces precede the abstract. The abstract
  % must be limited to one paragraph.

\begin{abstract}

The ocean is a crucial component of the Earth's system. 
It profoundly influences human activities and plays a critical role in climate regulation. 
Our understanding has significantly improved over the last decades with the advent of satellite remote sensing data, allowing us to capture essential sea surface quantities over the globe, e.g., sea surface height (SSH). 
Despite their ever-increasing abundance, ocean satellite data presents challenges for information extraction due to their sparsity and irregular sampling, signal complexity, and noise. 
Machine learning (ML) techniques have demonstrated their capabilities in dealing with large-scale, complex signals. 
Therefore we see an opportunity for these ML models to harness the full extent of the information contained in ocean satellite data. 
However, data representation and relevant evaluation metrics can be \textit{the} defining factors when determining the success of applied ML. 
The processing steps from the raw observation data to a ML-ready state and from model outputs to interpretable quantities require domain expertise, which can be a significant barrier to entry for ML researchers. 
In addition, imposing fixed processing steps, like committing to specific variables, regions, and geometries, will narrow the scope of ML models and their potential impact on real-world applications. 
\textbf{OceanBench} is a unifying framework that provides standardized processing steps that comply with domain-expert standards. 
It is designed with a flexible and pedagogical abstraction: it a) provides plug-and-play data and pre-configured pipelines for ML researchers to benchmark their models w.r.t. ML and domain-related baselines and b) provides a transparent and configurable framework for researchers to customize and extend the pipeline for their tasks. 
In this work, we demonstrate the \texttt{OceanBench} framework through a first edition dedicated to SSH interpolation challenges. 
We provide datasets and ML-ready benchmarking pipelines for the long-standing problem of interpolating observations from simulated ocean satellite data, multi-modal and multi-sensor fusion issues, and transfer-learning to real ocean satellite observations. 
The \texttt{OceanBench} framework is available at~\href{https://github.com/jejjohnson/oceanbench}{github.com/jejjohnson/oceanbench} and the dataset registry is available at~\href{https://github.com/quentinf00/oceanbench-data-registry}{github.com/quentinf00/oceanbench-data-registry}.

\end{abstract}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% - We demonstrate how \texttt{OceanBench} can be used as an underlying framework with a series of SSH interpolation tasks which combines different variables, regions and geometries. 


% Q - make use of everything we mentioned above!
% E/Q - we want to showcase that OceanBench can be used for SSH interpolation 
% - we want to demonstrate how we can design different experiments/modifications with minimal code changes
% Q - simple tasks SSH -> SSH; extend it a) add domain, b) include other variables, c) switching to real data
% - enrich a simple experimental setups with additional variations

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% - There is some work to be done to get the observation data to a ML-ready state.
% - Deciding the appropriate transformations requires domain-expertise which can be a large barrier to entry for ML researchers.

% - ML methods cannot be applied out of the box on raw observation data because .. blah blah

% - Despite the potential of machine learning to solve the issues that plague geosciences, the barrier to entry for machine learning (ML) researchers in ocean sciences is often hindered by the vastly different schemes for preprocessing techniques required to get the geo-centric data to a ML-ready state.
% \texttt{OceanBench} is a framework for co-designing machine learning-driven high level data products from ocean observations. 
%%%%%%%%%
% Why dont we just provide the processed data and call it a day...?
% Q - 1) non-standardized preprocessing steps; 2) regional differences
% 1 - multiple ways to take advantage of the Obs data (covariates, coordinate-based, gridded)
% Keeping the flexibilities allow for extensibility and multiple 
%%%%%%%%%%%%$
% 1 - OceanBench is a unifying framework that provides standardized processing steps that comply with domain-expert standards.
% 2 - It is designed for - flexible, padagological, abstract, :
% a - getting ML researchers quickly involved (data + preconfigured pipelines -> ML ready setups and test their models)
% - provides data and preconfigured pipelines for ML researchers to quickly experiment with different setups,
% - transparent and configurable for researchers to customize and extend the pipeline for their own objectives
% b - pedagological, unified setup to create and modified tasks (extensible)
% - flexibility
% 3 - We demonstrate ho
% %
% \texttt{OceanBench} is a framework that standardizing ... these processing steps that comply with domain-expert standards.
% %
% It is designed to lower the barrier to entry for ML researchers by providing preconfigured pipelines, ... "one-stop-shop for it all", and providing illustrative examples for different audiences.
% * 
% * provide a common interface for the processing steps
% * create a few ML tasks from raw data to ML ready using the above steps
% * showcase how one can orchestrate preconfigured pipelines to create a variety of ML tasks
% * preconfigured pipelines to illustrate example applications

% 1 - getting ML researchers quickly involved (data + preconfigured pipelines -> ML ready setups and test their models)
% 2 - pedagological, unified setup to create and modified tasks

% %%%%%
% \texttt{OceanBench} is a framework 
% - lower the barrier to entry
% - accessibility
% - one place to look to get all the stuff you want to do
% - preconfigured pipelines
% - jbooks with illustrated examples.
% - standardized preprocessing steps.
%
% It seeks to maintains readability, robustness, and flexibility by providing a standardized framework to explicitly highlight the preprocessing step used, the parameters chosen and the sequence of operations performed. 
%
% It takes a step towards incorporate these domain-driven decisions to integrate well with existing ML pipelines.
%
% We demonstrate the usefulness of \texttt{OceanBench} on a series of SSH interpolation tasks with 
% consistent dataflow pipelines, physically-inspired metrics, and interpretable visualizations.

==> content/1_motivation.tex <==
\section{Motivation}

The ocean is vital to the Earth's system~\cite{OCEANWARMING}. 
It plays a significant role in climate regulation regarding carbon~\cite{OCEANCARBONCYCLE} and heat uptake~\cite{OCEANHEATUPTAKE}. It is also a primary driver of human activities (e.g., maritime traffic and world trade, marine resources and services)~\cite{SSHOPERATIONAL, ML4OCN}. 
However, monitoring the ocean is a critical challenge: the ocean state can only partially be determined because most of the ocean consists of subsurface quantities that we cannot directly observe. 
Thus, to quantify even a fraction of the physical or biochemical ocean state, we must often rely only on surface quantities that we can monitor from space, drifting buoys, or autonomous devices.
Satellite remote sensing, in particular, is one of the most effective ways of measuring essential sea surface quantities~\cite{Altimetry} such as sea surface height (SSH)~\cite{DUACS}, sea surface temperature (SST)~\cite{OCEANSATELLITESST}, and ocean color (OC)~\cite{OCEANSATELLITEOC}. 
While these variables characterize only a tiny portion of the ocean ecosystem, they present a gateway to many other derived physical quantities~\cite{ML4OCN}.


% satellite-derived SSH data allow us to monitor the sea level rise as well as critical physical and biogeochemical ocean processes,
Although we can access observable sea surface quantities, they are generally irregularly and extremely sparsely sampled. 
For instance, satellite-derived SSH data has less than 5\% coverage of the globe daily~\cite{DUACS}. 
These sampling gaps make the characterization of ocean processes highly challenging for operational products and downstream tasks that depend on relevant gap-free variables. This has motivated a rich literature in geoscience over the last decades, mainly using geostatistical kriging methods \cite{DUACS, MIOST} and model-driven data assimilation schemes~\cite{BFNQG, GLORYS12}. Despite significant progress, these schemes often need to improve their ability to leverage available observation datasets' potential fully. 
This has naturally advocated for exploring data-driven approaches like shallow ML schemes~\cite{DINEOF, DINEOF2, ANALOGDA2, ANALOGDA}. Very recently, deep learning schemes \cite{SSHInterpAttention, SSHInterpConvLSTM, SSHInterpUNet} have become appealing solutions to benefit from existing large-scale observation and simulation datasets and reach significant breakthroughs in the monitoring of upper ocean dynamics from scarcely and irregularly sampled observations. However, the heterogeneity and characteristics of the observation data present major challenges for effectively applying these methods beyond idealized case studies. 
A data source could have different variables, geometries, and noise levels, resulting in many domain-specific preprocessing procedures that can vastly change the solution outcome.
Furthermore, the evaluation procedure of the methods and their effectiveness can be regionally-dependent as the physical phenomena vary in space and time, which adds another layer of complexity in convincing domain scientists of their trustworthiness.
So the entire ML pipeline now requires a unified framework for dealing with heterogeneous data sources, different pre- and post-processing methodologies, and regionally-dependent evaluation procedures.

 %So the nature of the observations presents a key challenge for operational products and downstream tasks that depend on relevant gap-free variables.
%In addition, this sparsity 
%Although methods like smoothers~\tocite{OI, MIOST}, data assimilation~\tocite{BFN} and machine learning (ML)~\tocite{NerFs,recent-stuff, Ronan} have produced viable solutions to filling the gaps in ocean satellite, the heterogeneity and characteristics of the observation data present major challenges for effectively applying these methods. 
% No model nor observation systems captures all scales and processes.
% Operational methods like optimal interpolation and data assimilation ...
% Thus, there is a need for better model/data integration schemes that fully benefit from HR models and ever-increasing observation datasets.

% \textbf{Opportunity}.
%An end-to-end framework for piping data from its raw form to an ML-ready state and from model outputs to interpretable quantities is challenging. Designing an effective system that does this is the basis for many MLOPs tools and research~\tocite{MLOPs Research}.
To address these challenges, we introduce \textbf{OceanBench}, a framework for co-designing machine-learning-driven high-level experiments from ocean observations. 
It consists of an end-to-end framework for piping data from its raw form to an ML-ready state and from model outputs to interpretable quantities. 
We regard \texttt{OceanBench} as a key facilitator for the uptake of MLOPs tools and research~\cite{MLOPS1,MLOPS2} for ocean-related datasets and case studies. This first edition provides datasets and ML-ready benchmarking pipelines for SSH interpolation problems, an essential topic for the space oceanography community, related to ML communities dealing with issues like in-painting~\cite{InPaintingSurvey}, denoising~\cite{DENOISESURVEY,DENOISESURVEY2}, and super-resolution~\cite{SuperResSurvey}. 
We expect \texttt{OceanBench} to facilitate new challenges to the applied machine learning community and contribute to meaningful ocean-relevant breakthroughs.
%
The remainder of the paper is organized as follows: in \S2, we outline some related work that was inspirational for this work; in \S3, we formally outline \texttt{OceanBench} by highlighting the target audience, code structure, and problem scope; in \S4, we outline the problem formulation of SSH interpolation and provide some insight into different tasks related to SSH interpolation where \texttt{OceanBench} could provide some helpful utility; and in \S5 we give some concluding remarks while also informally inviting other researchers to help fill in the gaps.

% \textbf{How We Measure SSH + Gap Problem}. 




% % \textbf{Data Deluge, Gaps, \& ML Integration}. 
% Like most geosciences, the ocean sciences also suffer from the data deluge that persists due to the large amounts of observed quantities being collected daily~\tocite{Gus}. 
% The increased availability and quantity of observations are beneficial because it offers the community more insight into the physical processes at a finer resolution.
% % Consequently, this can help oceanographers revolve a central question of observing and predicting the ocean state at different spatial and timescales. 
% The trade-off is that processing this data is very expensive.
% Furthermore, it is impossible to accurately measure the entire globe concurrently, resulting in data with many gaps.
% Many operational systems have historically used ad-hoc coordinate-based schemes to gap-fill the data based on covariance assumptions. 
% However, with the abundance of new data~\tocite{SWOT}, these covariance-based schemes are reaching their limit due to the computational and signal complexity.
% Machine learning (ML) has been recently introduced as a viable alternative to filling the gaps in data where many classes of methods have found success, including coordinate-based methods~\tocite{OI,MIOST,NerFs}, direct surrogate/hybrid methods~\tocite{BFN, recent-stuff}, and end-to-end learning schemes~\tocite{Ronan}. 
% Nevertheless, most of these methods have only been applied to regions, and more needs to be applied at a large scale that comes close to the operational settings.


% % \textbf{Logistics Problem}.
% % \textbf{The Problem with Observation Data}.
% % The community is quickly facing a logistics problem.
% Dealing with complex problems such as SSH interpolation requires dealing directly with the observation data, often involving aggregating observations from satellites, buoys, or autonomous devices.
% In all cases, we can only observe a tiny portion of the Earth at any given time, resulting in highly sparse data (often <5\% coverage).
% This problem is even more difficult because the data sources are often heterogeneous, with different variables, geometries, and noise levels.
% Furthermore, the evaluation procedure can be regionally dependent as the physical phenomena vary globally. 
% So the entire ML pipeline now requires a unified framework for dealing with heterogeneous data sources, different pre- and post-processing methodologies, and regional dependent evaluation procedures.

% To solve a difficult problem such as SSH interpolation requires a lot of interdisciplinary expertise including scientific, numerical and machine learning.
% To do effective ML research in this area, one needs a consistent \textit{pipeline} to funnel the data from its raw form through the transformations and to its evaluation state. 
% In standard ML research, we have copious amounts of \textit{datamodules} which encapsulate many underlying transformations procedures for many staple datasets, e.g. MNIST, CIFAR10, CELEB, etc.
% Even some weather and climate benchmark datasets have \cite{weatherbench,ClimateBench} access to gap-free, non-heterogenous reanalysis data.
% Despite the focus on the ML model in the current state of affairs, we have often found that the variables chosen and how they were preprocessed has the greatest effect on the final result.
% In previous benchmark settings~\citep{CHAOSBENCH,PDEBench,ClimateBench,weatherbench,ENS10Bench}, little attention was paid to the internals of the data preprocessing and this process was kept static.
% In geosciences, because we often deal with sparse, heterogeneous observations, we often need to decide and implement many crucial preprocessing transformations before we get to the modeling aspects.
% % including selecting regions, filtering, and calculating derived variables.
% As such, we should include the chosen variables and how they are preprocessed as hyperparameters to be optimized within the full ML pipeline.
% However, this complicates the entire pipeline because we have effectively compounded the complexity due to the many ways one can preprocess and modify the data in conjunction with decisions from the ML side like the architecture, the optimizer and the loss function.
% In addition, we may even have a large series of post-processing transformations which determine how we evaluate our models. Those transformations contain implementation details that may change between studies which make comparing and reproducing some results challenging.
% This results in a software engineering (SWE) roadblock which needs to be addressed should we wish to do effective research in applied ML research and this obstacle is especially prevalent in the geosciences.



% , through the transformations, into the model, and through the 
% Due to many of the many components needed to solve the problem it requires a pipeline. 
% For domain scientists, there is a lack of organization and ontology of previous ideas. 
% For machine learning researchers, ... 
% For downstream users, there is a lack of ontology of the current state of research which makes it difficult to readily apply these techniques for their problems.

% Nonetheless, most of this research has been done in parallel across disjoint sub-fields of research and to the best of our knowledge little to no work has been done on homogenising and integrating these distinct methods in a common framework



% In this paper, we wish to establish a well-defined software abstraction for dealing SSH interpolation using ML.
% Using ocean data is the primary goal which is a data assimilation problem. 
% However, there are many subsequent steps we need to improve. 1) We need gap-free data from the satellite observations, 2) we need surrogate or hybrid models to replace the expensive ocean models, and 3) we need end-to-end learning schemes to perform domain-specific tasks that incorporate good priors and the observations.


==> content/2_related_work.tex <==
\section{Related Work}

Machine learning applied to geosciences is becoming increasingly popular, but there are few examples of transparent pipelines involving observation data. 
After a thorough literature review, we have divided the field into three camps of ML applications that pertain to this work: 1) toy simulation datasets, 2) reanalysis datasets, and 3) observation datasets. 
We outline the literature for each of the three categories below.

\textbf{Toy Simulation Data}. 
One set of benchmarks focuses on learning surrogate models for well-defined but chaotic dynamical systems in the form of ordinary differential equations (ODEs) and partial differential equations (PDEs) and there are freely available code bases which implement different ODEs/PDEs~\citep{CHAOSBENCH,PDEBench,pyQG,JAXCFD,NCARDART,NCARDARTSOFTWARE,VEROS,OCEANANIGANS}.
% For example, \texttt{Dyst} package~\cite{CHAOSBENCH} has many chaotic ODEs, and packages such as \texttt{PDEBench}~\cite{PDEBench}, pyQG~\citep{pyQG}, NCAR DART~\citep{NCARDART,NCARDARTSOFTWARE}, and jax-CFD~\citep{JAXCFD} have implementations of 2D/3D Spatial-Temporal PDEs similar to Navier-Stokes; 
This is a great testing ground for simple toy problems that better mimic the structures we see in real-world observations. 
% More ocean-related simulations include the pyQG package~\citep{pyQG}, the NCAR DART data assimilation testbed~\citep{NCARDART,NCARDARTSOFTWARE}.
Working with simulated data is excellent because it is logistically simple and allows users to test their ideas on toy problems without increasing the complexity when dealing with real-world data.
However, these are ultimately simple physical models that often do not reflect the authentic structures we see in real-world, observed data.

\textbf{Reanalysis Data}. 
This is assimilated data of real observations and model simulations. 
There are a few major platforms that host ocean reanalysis data like the Copernicus Marine Data Store~\citep{MDSOCEANPHYSICS,MDSBIOGEOCHEMICAL,MDSOCEANPHYSICSENS,MDSWAVES}, the Climate Data Store~\citep{CDSREANALYSISSST}, the BRAN2020 Model~\citep{DATABLUELINK}, and the NOAA platform~\citep{DATANCEP}. 
However, to our knowledge, there is no standard ML-specific ocean-related tasks to accompany the data. On the atmospheric side, platforms like \texttt{WeatherBench}~\cite{weatherbench}, \texttt{ClimateBench}~\cite{ClimateBench}, \texttt{ENS10}~\cite{ENS10Bench} were designed to assess short-term and medium-term forecasting using ML techniques with recent success of ML~\cite{GraphCast,FourCastNet}
% While the original papers featured straightforward methods, there has been swift subsequent development within the last few years~\cite{GraphCast,FourCastNet}. 
% Apart from industry momentum and investment, we attribute the recent adoption and success of ML to the problem's clarity, the original tasks' openness, and the software's ML compatibility. 
The clarity of the challenges set by the benchmark suites has inspired the idea of \texttt{OceanBench}, where we directly focus on problems dealing with ocean observation data.

\textbf{Observation Data}. 
These observation datasets (typically sparse) stem from satellite observations that measure surface variables or in-situ measurements that measure quantities within the water column. 
Some major platforms to host data include the Marine Data Store~\citep{MDSALONGTRACK,MDSINSITU}, the Climate Data Store~\citep{CDSOBSSST,CDSOBSSSTENS,CDSOBSOC}, ARGO~\citep{ARGO}, and the SOCAT platform~\citep{SOCAT}.
However, it is more difficult to assess the efficacy of operational ML methods that have been trained only on observation data and, to our knowledge, there is no coherent ML benchmarking system for ocean state estimation.
% In one community, there is the Surface Ocean CO$_2$ Atlas (SOCAT)~\cite{SOCAT} which is a community effort to aggregate all collocated observations (included SSH) which help predict the fugacity of carbon dioxide (fCO$_2$). 
% This has been a huge effort to provide a consistently updated suite of observations for some key variables that are important in biogeochemical processes.
% However, there is currently no coherent benchmarking system with standard metrics despite their being a wide range of new methods to try and tackle the interpolation problem.
% Most new work tends to use the observations provided with their own additional variable with no standard comparison framework other works.
% In a completely different community, 
There has been significant effort by the \textit{Ocean-Data-Challenge} Group\footnote{Ocean Data Challenge group: Freely associated scientist for oceanographic algorithm and product improvements (\href{https://ocean-data-challenges.github.io/}{ocean-data-challenges.github.io})} which provides an extensive suite of datasets and metrics for SSH interpolation.
% Their motivation is to investigate which methods could be employed for the upcoming SWOT mission~\cite{SWOT} which is highly-challenging for current operational interpolation techniques.
% where they provide over eight challenges of varying degrees of difficulty with completely open-source data, along with tutorials for metrics.
Their efforts heavily inspired our work, and we hope that \texttt{OceanBench} can build upon their work by adding cohesion and facilitating the ease of use for ML research and providing a high-level framework for providing ML-related data products.





==> content/3_oceanbench.tex <==
\section{OceanBench} \label{sec:oceanbench_intro}

\subsection{Why OceanBench?} \label{sec:oceanbench_why}

There is a high barrier to entry in working with ocean observations for researchers in applied machine learning as there are many processing steps for both the observation data and the domain-specific evaluation procedures. 
\texttt{OceanBench} aims to lower the barrier to entry cost for ML researchers to make meaningful progress in the field of state prediction. 
We distribute a standardized, transparent, and flexible procedure for defining data and evaluation pipelines for data-intensive geoscience applications. 
Proposed examples and case studies provide a plug-and-play framework to benchmark novel ML schemes w.r.t.  state-of-the-art, domain-specific ML baselines. 
In addition, we adopt a pedagogical abstraction that allows users to customize and extend the pipelines for their specific tasks.
To our knowledge, no framework embeds processing steps for earth observation data in a manner compatible with MLOps abstractions and standards regarding reproducibility and evaluation procedures. 
Ultimately, we aim to facilitate the uptake of ML schemes to address ocean observation challenges and to bring new challenges to the ML community to extend additional ML tools and methods for irregularly-sampled and partially-observed high-dimensional space-time dynamics.
The abstractions proposed here apply beyond ocean sciences and SSH interpolation to other geosciences with similar tasks that intersect with machine learning.

% \begin{itemize}
%     \item Establish a rigorous ontology of pre-, geo- and ML processing tools.
%     \item Consistent problems with detailed introductory tutorials
%     \item aggregate benchmarks with common tools
%     \item \textit{what i wish I had when i started this problem}
%     \item \textit{A lot of research gets lots in grad students laptops}
%     \item provide training, context and awareness to the different packages that exist to solve problems.
% \end{itemize}



\subsection{Code Structure} \label{sec:code_structure}

\texttt{OceanBench} is lightweight in terms of the core functionality.
We keep the code base simple and focus more on how the user can combine each piece.
We adopt a strict functional style because it is easier to maintain and combine sequential transformations. 
There are five features we would like to highlight about \texttt{OceanBench}: 1) Data availability and version control, 2) an agnostic suite of geoprocessing tools for \texttt{xarray} datasets that were aggregated from different sources,  3) Hydra integration to pipe sequential transformations, 4) a flexible multi-dimensional array generator from \texttt{xarray} datasets that are compatible with common deep learning (DL) frameworks, and 5) a JupyterBook~\cite{JupyterBook} that offers library tutorials and demonstrates use-cases.
In the following section, we highlight these components in more detail.

\textbf{Data Availability}. 
The most important aspect is the public availability of the datasets. 
We aggregate all pre-curated datasets from other sources, e.g. the \textit{Ocean-Data-Challenge}~\cite{DCOSEGULFSSH,DCOSSEGULFSSH}, and organize them to be publicly available from a single source~\footnote{Available at: \href{https://github.com/quentinf00/oceanbench-data-registry}{oceanbench-data-registry.github.com}}. 
We also offer a few derived datasets which can be used for demonstrations and evaluation. 
Data is never static in a pipeline setting, as one can have many derived datasets which stem from numerous preprocessing choices. 
In fact, in research, we often work with derived datasets that have already been through some preliminary preprocessing methods. 
To facilitate the ever-changing nature of data, we use the Data Version Control (\texttt{DVC}) tool~\cite{DVC}, which offers a git-like version control of the datasets.

\textbf{Geoprocessing Tools}. 
The core \texttt{OceanBench} library offers a suite of functions specific to processing geo-centric data. 
While a few particular functionalities vary from domain to domain, many operations are standard, e.g., data variable selections, filtering/smoothing, regridding, coordinate transformations, and standardization. 
We almost work exclusively with the \texttt{xarray}~\cite{XARRAY} framework because it is a coordinate-aware, flexible data structure. 
In addition, the geoscience community has an extensive suite of specialized packages that operate in the \texttt{xarray} framework to accomplish many different tasks. 
% A non-exhaustive, highlighted list of packages that are compatible with the \texttt{xarray} data structure include: \texttt{xgcm} for non-uniform grid operators, \texttt{pint} for unit-aware operators, \texttt{metpy} for gradient-based calculations, \texttt{pyinterp} and \texttt{xesmf} for advanced regridding methods, \texttt{xrft} and \texttt{xwavelet} for power spectrum analysis, \texttt{gcm-filters} for advanced filtering methods, and the \texttt{dask} suite for scaling everything to multi-core/node HPC environments. 
Almost all \texttt{OceanBench} toolsets are exclusively within the \texttt{xarray} framework to maintain compatibility with a large suite of tools already available from the community.


% As an ML practicioner navigating this sea of libraries can be intimidating as they require different input formats and domain specific parameters. Oceanbench aims at simplifying the use of these libraries by providing the necessary formatting tools and default usage of the different utilities.  

% There are many packages that exist independently which accomplish many of the specific tasks that most geoscientists need. 

\textbf{Hydra Integration}. 
As discussed above, many specific packages accomplish many different tasks. 
However, what needs to be added is the flexibility to mix and match these operations as the users see fit. 
\texttt{Hydra}~\cite{Hydra} provides a configurable way to aggregate and \textit{pipe} many sequential operations together. 
It also maintains readability, robustness, and flexibility through the use of \texttt{.yaml} files which explicitly highlights the function used, the function parameters chosen, and the sequence of operations performed. 
In the ML software stack, \texttt{Hydra} is often used to manage the model, optimizer, and loss configurations which helps the user experiment with different options. 
We apply this same concept in preprocessing, geoprocessing, and evaluation steps, often more important than the model configuration in geoscience-related tasks.  

\texttt{XRPatcher}~\footnote{Available at: \href{https://github.com/jejjohnson/xrpatcher/}{github.com/jejjohnson/xrpatcher}}. 
Every machine learning pipeline will inevitably require moving data from the geo-specific data structure to a multi-dimensional array easily digestible for ML models. 
A rather underrated, yet critical, feature of ML frameworks such as \texttt{PyTorch}~\cite{PYTORCH} (\texttt{Lightning}~\cite{LIGHTNING}) and \texttt{TensorFlow}~\cite{TENSORFLOW} (\texttt{Keras}~\cite{KERAS}) is the abstraction of the dataset, dataloader, datamodules, and data pipelines. 
In applied ML in geosciences, the data pipelines are often more important than the actual model~\cite{DATA4ML}. 
The user can control the \textit{patch}-size and the \textit{stride}-step, which can generate arbitrary coordinate-aware items directly from the \texttt{xarray} data structure. 
In addition, \texttt{XRPatcher} provides a way to reconstruct the fields from an arbitrary patch configuration.
This robust reconstruction step is convenient to extend the ML inference step where one can reconstruct entire fields of arbitrary dimensions beyond the training configuration, e.g., to account for the border effects within the field (see appendix~\ref{sec:xrpatcher}) or to reconstruct quantities in specific regions or globally. 

\textbf{JupyterBook}.
% ~\footnote{Available at: \href{https://jejjohnson.github.io/oceanbench/content/overview.html}{jejjohnson.github.io/oceanbench}}. 
Building a set of tools is relatively straightforward; however, ensuring that it sees a broader adoption across a multi-disciplinary community is much more challenging. 
We invested heavily in showing use cases that appeal to different users with the \texttt{JupyterBook} platform~\cite{JupyterBook}. 
Code with context is imperative for domain and ML experts as we need to explain and justify each component and give many examples of how they can be used in other situations. 
% \texttt{Hydra} is an effective tool, but it has a steep learning curve, and the tutorials are very computer science-oriented, and there are many domain scientists (and seasoned ML researchers) who will. 
Thus, we have paid special attention to providing an extensive suite of tutorials, and we also highlight use cases for how one can effectively use the tools. 


\subsection{Problem Scope} \label{sec:problem_scope}

% As outlined in the introduction, we are interested in the state estimation problem for important variables like SSH and SST. We use the data assimilation perspective whereby state estimation is defined as the combination of observations, constraints and initial state~\citep{DAGEOSCIENCE}. Tackling the issue of state estimation directly is very challenging due to the uncertainty in the measurements, the prior constraints, and the initial state. In addition, there are many logistical constraints that further complicate the problem including the very high-dimensional, spatiotemporal state space, the multi-scale complexity of the dynamics, and the extreme missing data.




There are many problems that are of great interest the ocean community~\citep{ML4DA} but we limit the scope to state estimation problems~\citep{DAGEOSCIENCE}. Under this scope, there are research questions that are relevant to operational centers which are responsible for generating the vast majority of global ocean state maps~\citep{MDSOCEANPHYSICS,MDSOCEANPHYSICSENS,MDSBIOGEOCHEMICAL, MDSWAVES} that are subsequently used for many downstream tasks~\citep{ML4OCN}. For example: how can we effectively use heterogeneous observations to predict the ocean state on the sea surface~\citep{BFNQG,NERFSSSH,MIOST,4DVARNETSST,4DVARNETSWOT,OCEANSATELLITESST}; how can we incorporate prior physics knowledge into our predictions of ocean state trajectories~\citep{BFNQG,ML4DA,ML4OCN}; and how can we use the current ocean state at time $T$ to predict the future ocean state at time $T+\tau$~\citep{METNET2,weatherbench,FORECASTSSCGP}.
In the same vain, there are more research questions that are of interest to the academic modeling community. For example: is simulated or reanalysis data more effective for learning ML emulators that replace expensive ocean models~\citep{MLSUBGRID,MLCLOSURE}; what metrics are more effective for assessing our ability to mimic ocean dynamics~\citep{SSTFLOWANOMALY,MLMETRICSINVARIANCE}; and how much model error can we characterize when learning from observations~\citep{MLMODELERR,MLMODELERR2}. 

We have cited many potential applications of how ML can be applied to tackle the state estimation problem. 
However, to our knowledge there is no publicly available, standardized benchmark system that is caters to ML-research standards.
We believe that, irrespective of the questions posed above and the data we access, there are many logistical similarities for each of the problem formulations where we can start to set standards for a subset of tasks like interpolation or forecasting. 
On the front-end, we need a way to select regions, periods, variables, and a valid train-test split (see sec. ~\ref{sec:hydra_recipe_task}). 
On the back-end, we need a way to transform the predictions into more meaningful variables with appropriate metrics for validation (see sec. ~\ref{sec:hydra_geoprocess_task} and ~\ref{sec:hydra_evaluation_task}).
\texttt{OceanBench} was designed to be an agnostic tool that is extensible to the types of datasets, processing techniques and metrics needed for working with a specific class of Ocean-related datasets. 
We strongly feel that a suite like this is the first step in designing task-specific benchmarks within the ocean community that is compatible with ML standards. 
In the remainder of the paper, we will demonstrate how \texttt{OceanBench} can be configured to facilite a ML-ready data challenge involving our first edition to demonstrate \texttt{OceanBench}'s applicability: sea surface height interpolation.


==> content/4_tasks.tex <==
\section{\textit{Sea Surface Height Edition}}\label{sec:interp_challenge}

Sea surface height (SSH) is one of the most critical, observable quantities when determining the ocean state. 
It is widely used to study ocean dynamics and the adverse impact on global climate and human activities~\cite{SSHMESOSCALE}. 
SSH enables us to track phenomena such as currents and eddies~\cite{SSHMESOSCALE,SSHMESOSCALE2,SSHMESOSCALE3}, which leads to a better quantification of the transport of energy, heat, and salt. 
In addition, SSH helps us quantify sea level rise at regional and global scales~\cite{SSHSEALEVEL,OCEANSEALEVEL}, which is used for operational monitoring of the marine environment~\cite{SSHOPERATIONAL}. 
Furthermore, SSH characterization provides a plethora of data products that downstream tasks can use for many other applications~\cite{SSH3DCIRCULATION, 3DQGOC}.
%
Due to the irregular sampling delivered by satellite altimeter, state-of-the-art operational methods using optimal interpolation schemes~\cite{DUACS, MIOST} or model-driven data assimilation~\cite{DINEOF, DINEOF2, ANALOGDA, ANALOGDA2} fail to fully retrieve SSH dynamics at fine scales below 100-200km on a global or regional scale, so improving the space-time resolution of SSH fields has been a critical challenge in ocean science. 
Beyond some technological developments~\cite{SWOT}, recent studies support the critical role of ML-based schemes in overcoming the current limitations of the operational systems~\cite{4DVARNETSWOT, BFNQG, SSHInterpAttention} .  
%
The rest of this section gives an overview of the general problem definition for SSH interpolation, followed by a brief ontology for ML approaches to address the problem. 
We also give an overview of some experimental designs and datasets with a demonstration of metrics and plots generated by the \texttt{OceanBench} platform. 



\subsection{Problem Definition}\label{sec:prob_definition}

We are dealing with satellite observations, so we are interested in the domain across the Earth's surface. 
Let us define the Earth's domain by some spatial coordinates, $\mathbf{x} = [\text{Longitude},\text{Latitude}]^\top \in\mathbb{R}^{D_s}$, and temporal coordinates, $t=[\text{Time}]\in\mathbb{R}^+$, where $D_s$ is the dimensionality of the coordinate vector.  
We can define some spatial (sub-)domain, $\Omega\subseteq\mathbb{R}^{D_s}$, and a temporal (sub-)domain, $\mathcal{T}\subseteq\mathbb{R}^+$. 
This domain could be the entire globe for 10 years or a small region within the North Atlantic for 1 year.
\begin{align}  \label{eq:spatiotemporal_coords}
    \text{Spatial Coordinates}: && \mathbf{x} &\in \Omega \subseteq \mathbb{R}^{D_s}\\ 
    \text{Temporal Coordinates}: && t &\in \mathcal{T} \subseteq \mathbb{R}^+.
\end{align}
In this case $D_s=2$ because we only have a two coordinates, however we can do some coordinate transformations like spherical to Cartesian. Likewise, we can do some coordinate transformation for the temporal coordinates like cyclic transformations or sinusoidal embeddings~\cite{ATTENTION}. We have two fields of interest from these spatiotemporal coordinates: the state and the observations.
\begin{align} \label{eq:state_obs}
    \text{State}: && \boldsymbol{u}(\mathbf{x},t) &: \Omega\times\mathcal{T}\rightarrow\mathbb{R}^{D_u} \\
    \text{Observations}: && \boldsymbol{y}_{obs}(\mathbf{x},t) &: \Omega\times\mathcal{T}\rightarrow\mathbb{R}^{D_{obs}}
\end{align}
The state domain, $u\in\mathcal{U}$, is a scalar or vector-valued field of size $D_u$ which is typically the quantity of interest and the observation domain, $y_{obs}\in\mathcal{Y}_{obs}$, is the observable quantity which is also a scalar or vector-valued field of size $D_{obs}$. Now, we make the assumption that we have an operator $\mathcal{H}$ that transforms the field from the state space, $\boldsymbol{u}$, to the observation space, $\boldsymbol{y}_{obs}$.
\begin{align} \label{eq:prob_definition}
    \boldsymbol{y}_{obs}(\mathbf{x},t) = \mathcal{H}\left(\boldsymbol{u}(\mathbf{x},t), t, \boldsymbol{\varepsilon}, \boldsymbol{\mu}\right) 
\end{align}
This equation is the continuous function defined over the entire spatiotemporal domain.  
The operator, $\mathcal{H}(\cdot)$, is flexible and problem dependent.
For example, in a some discretized setting there are 0's wherever there are no observations, and 1's wherever there are observations, and in other discretized settings it takes a weighted average of the neighboring pixels.
We also include a generic noise function, $\boldsymbol{\varepsilon}(\mathbf{x},t)$.
This could stem from a distribution, it could stationary noise operator, $\boldsymbol{\varepsilon}(\mathbf{x})$, or it could be constant in space but vary with Time, $\boldsymbol{\varepsilon}(t)$. 
We also include a control parameter, $\boldsymbol{\mu}$, representing any external factors or latent variables that could connect the state vector to the observation vector, e.g., sea surface temperature.
%
%###########################################################################################
%
% CAN BE FRAMED AS INVERSE PROBLEMS
%
Our quantity of interest is SSH, $\eta$, a scalar-valued field defined everywhere on the domain. In our application, we assume that the SSH we observe from satellite altimeters, $\eta_{obs}$, is the same as the SSH state, except it could be missing for some coordinates due to incomplete coverage from the satellite. So our transformation is defined as follows:
\begin{align} \label{eq:ssh_field_continuous}
\boldsymbol{\eta}_{obs}(\mathbf{x},t) &= \mathcal{H}\left(\boldsymbol{\eta}(\mathbf{x},t), t, \boldsymbol{\varepsilon}, \boldsymbol{\mu}\right)
% , \hspace{10mm}
% \mathbf{x} \in \Omega \subseteq \mathbb{R}^{D_s}, \hspace{10mm} 
% t \in \mathcal{T} \subseteq \mathbb{R}^+.
\end{align}
In practice, the satellite providers have a reasonable estimation of the amount of structured noise level we can expect from the satellite altimetry data; however, unresolved noise could still be present. 
% Although we do not explicitly specify the control parameter, $\boldsymbol{\mu}$, we leave it into the equation to account for any other state parameters not accounted for in our model. 
Finally, we are interested in finding some model, $\mathcal{M}$, that maps the SSH we observe to the true SSH given by
\begin{align} \label{eq:interp_problem}
    \mathcal{M} &: \boldsymbol{\eta}_{obs}(\mathbf{x}, t, \boldsymbol{\mu}) \rightarrow \boldsymbol{\eta}(\mathbf{x},t),
%     , \hspace{10mm}
% \mathbf{x} \in \Omega \subseteq \mathbb{R}^{D_s}, \hspace{10mm} 
% t \in \mathcal{T} \subseteq \mathbb{R}^+.
\end{align}
which is essentially an inverse problem that maps the observations to the state.
One could think of it as trying to find the inverse operator, $\mathcal{M}=\mathcal{H}^{-1}$, but this could be some other arbitrary operator.  
%
\subsection{Machine Learning Model Ontology} \label{sec:ml_ontology_mini}

In general, we are interested in finding some parameterized operator, $\mathcal{M}_{\boldsymbol{\theta}}$, that maps the incomplete SSH field to the complete SSH field
\begin{align} \label{eq:ml_interp_problem}
    \mathcal{M}_{\boldsymbol{\theta}} &: \boldsymbol{\eta}_{obs}(\mathbf{x}, t, \boldsymbol{\mu}) \rightarrow \boldsymbol{\eta}(\mathbf{x},t),
\end{align}
whereby we learn the parameters from data.
%
The two main tasks we can define from this problem setup are 1) interpolation and 2) extrapolation.
We define \textit{interpolation} as the case when the boundaries of the inferred state domain lie within a predefined shape for the boundaries of the spatiotemporal observation domain. 
For example, the shape of the spatial domain could be a line, box, or sphere, and the shape of the temporal domain could be a positive real number line.
We define \textit{extrapolation} as the case where the boundaries of the inferred state domain are outside the boundaries of the spatiotemporal observation domain. 
In this case, the inferred state domain could be outside of either domain or both. 
A prevalent specific case of extrapolation is \textit{hindcasting} or \textit{forecasting}, where the inferred state domain lies within the spatial observation domain's boundaries but outside of the temporal observation domain's.
In the rest of this paper, we will look exclusively at the interpolation problem. 
However, we refer the reader to appendix~\ref{sec:other_tasks} for a more detailed look at other subtasks that can arise.

From a ML point of view, we can explore various ways to define the operator in equation~\eqref{eq:interp_problem}. 
We may distinguish three main categories: (i) coordinate-based methods that learn a parameterized continuous function to map the domain coordinates to the scalar values, (ii) the explicit mapping of the state from the observation, (iii) implicit methods defined as the solution of an optimization problem. 
The first category comprises of kriging approaches, which have been used operationally with historical success~\cite{KRIGINGREVIEW,DUACS}. Beyond such covariance-based approaches, recent contributions explore more complex trainable functional models~\cite{GPsBIGDATA}, basis functions~\cite{MIOST}, and neural networks~\cite{NERFSSSH}. 
The second category of schemes bypasses the physical modeling aspect and amortizes the prediction directly using state-of-the-art neural architectures such as UNets and ConvLSTMs~\cite{SSHInterpAttention, SSHInterpConvLSTM, SSHInterpUNet}. 
This category may straightforwardly benefit from available auxiliary observations~\citep{CDSOBSSST,CDSOBSSSTENS,CDSOBSOC} 
% (including available operational gap-free SST products~\citep{CDSOBSSST,CDSOBSSSTENS} and other sea surface quantities~\citep{CDSOBSOC})
to state the interpolation problem as a super-resolution~\cite{SuperResSurvey} or image-to-image translation problem~\cite{IMAGE2IMAGETRANSLATION, IMAGE2IMAGETRANSLATION2}. 
The third category relates to inverse problem formulations and associated deep learning schemes, for example deep unfolding methods and plug-and-play priors~\cite{DEEPUNFOLDING}. 
Interestingly, recent contributions explore novel neural schemes which combine data assimilation formulations~\cite{DAGEOSCIENCE} and learned optimizer strategies~\cite{4DVARNETSWOT,4DVARNETSST}.
We provide a more detailed ontology of methods used for interpolation problems in appendix~\ref{sec:ml_ontology}. 
We consider at least one baseline approach from each category for each data challenge described in section~\ref{sec:data_challenges}. 
While all these methods have pros and cons, we expect the OceanBench platform to showcase to new experimental evidence and understanding regarding their applicability to SSH interpolation problems.
 

\subsection{Experimental Design} \label{sec:experimental_design}

\begin{table}[ht]
\caption{This table gives a brief overview of the datasets provided to complete the data challenges listed in~\ref{sec:data_challenges} and~\ref{sec:data_challenges_extended}. Note that the OSSE datasets are all gridded products whereas the OSE NADIR is an alongtrack product. See figure~\ref{fig:oceanbench_maps} for an example of the OSSE NEMO Simulations for SSH and SST and pseudo-observations for NADIR \& SWOT.}
\label{tb:datasets}
\centering
\begin{tabular}{lcccc}
 \toprule
 & OSSE & OSSE NADIR + SWOT & OSSE SST & OSE NADIR  \\ \midrule
 Data Type & Simulations & 
Pseudo-Observations & 
 Simulations & Observations \\
Source     & 
NEMO~\citep{NEMOAJAYI2020} & 
NEMO~\citep{NEMOAJAYI2020} &
NEMO~\citep{NEMOAJAYI2020}
% \multicolumn{3}{c}{NEMO GCM\citep{NEMOAJAYI2020}}  
& Altimetry~\citep{MDSALONGTRACK} \\
Region & 
GulfStream & GulfStream & GulfStream & GulfStream \\
Domain Size &
% ($L_x\times L_y$) 
$10\times 10^\circ$ &
$10\times 10^\circ$ &
$10\times 10^\circ$ &
$10\times 10^\circ$
\\
Longitude Extent &
$[-65^\circ, -55^\circ]$ & 
$[-65^\circ, -55^\circ]$ &
$[-65^\circ, -55^\circ]$ &
$[-65^\circ, -55^\circ]$ \\
Latitude Extent &
$[33^\circ, 43^\circ]$ &
$[33^\circ, 43^\circ]$ &
$[33^\circ, 43^\circ]$ &
$[33^\circ, 43^\circ]$ \\
Resolution &
% ($\Delta_x\times \Delta_y$) 
$0.05^\circ\times 0.05^\circ$ &
$0.05^\circ\times 0.05^\circ$ &
$0.05^\circ\times 0.05^\circ$ &
$7$ km \\
Grid Size &
$200\times 200$ & $200\times 200$ & $200\times 200$ & N/A \\
Num Datapoints &
$\sim$14.6M & $\sim$14.6M & $\sim$14.6M & $\sim$1.6M \\
Period Start & 2012-10-01 & 2012-10-01 & 2012-10-01 & 2016-12-01 \\
Period End & 2013-09-30 & 2013-09-30 & 2013-09-30 & 2018-01-31 \\
Frequency  & Daily & Daily & Daily & 1 Hz \\
\bottomrule
\end{tabular}
\end{table}

The availability of multi-year simulation and observation datasets naturally advocates for the design of synthetic (or twin) experiments, referred to as observing system simulation experiments (OSSE), and of real-world experiments, referred to as observing system experiments (OSE).
We outline these two experimental setups below.

\textbf{Observing System Simulation Experiments (OSSE)}. A staple and groundtruthed experimental setup uses a reference simulation dataset to simulate the conditions we can expect from actual satellite observations. 
This setup allows researchers and operational centers to create a fully-fledged pipeline that mirrors the real-world experimental setting.
An ocean model simulation is deployed over a specified spatial domain and period, and a satellite observation simulator is deployed to simulate satellite observations over the same domain and period. 
This OSSE setup has primarily been considered for performance evaluation, as one can assess a reconstruction performance over the entire space-time domain. It also provides the basis for the implementation of classic supervised learning strategies~\cite{SSHInterpUNet,SSHInterpConvLSTM,SSHInterpAttention}.
The domain expert can vary the experimental conditions depending on the research question. 
For example, one could specify a region based on the expected dynamical regime~\cite{DCOSSEGULFSSH} or add a certain noise level to the observation tracks based on the satellite specifications.
The biggest downside to OSSE experiments is that we train models exclusively with ocean simulations which could produce models that fail to generalize to the actual ocean state. 
Furthermore, the simulations are often quite expensive, which prevents the community from having high spatial resolution over very long periods, which would be essential to capture as many dynamical regimes as possible.


\begin{figure}[t!]
\small
\begin{center}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccc}
NADIR Altimetry Tracks & 
SWOT Altimetry Tracks &
Sea Surface Temperature \\
\includegraphics[width=42.5mm, height=30mm]{content/figures/maps/sla/dc20a_ssh_anomaly_nadir4_20121027.png} 
% \includegraphics[bb=0 0 4 3]{content/figures/maps/sla/dc20a_ssh_anomaly_nadir4_20121027.png} 
&
\includegraphics[width=42.5mm, height=30mm]{content/figures/maps/sla/dc20a_ssh_anomaly_swot1nadir5_20121027.png} &
\includegraphics[width=4.25cm,height=3cm]{content/figures/maps/sst/dc20a_nemo_sst.png}
\end{tabular}
\begin{tabular}{cccc}
\hspace{3mm} NEMO Simulation & 
\hspace{3mm} MIOST & 
\hspace{3mm} BFNQG & 
4DVarNet \\
\vspace{-2mm}
%%%%% SEA LEVEL ANOMALY %%%%%%%%
\includegraphics[trim={0 0 42mm 0},clip, width=3.20cm,height=3cm]{content/figures/maps/sla/dc20a_nemo_sla.png} &
\includegraphics[trim={0 0 42mm 0},clip, width=3.2cm,height=3cm]{content/figures/maps/sla/dc20a_miost_sla.png} &
\includegraphics[trim={0 0 42mm 0},clip, width=3.2cm,height=3cm]{content/figures/maps/sla/dc20a_bfnqg_sla.png} &
\includegraphics[width=4.0cm,height=3cm]{content/figures/maps/sla/dc20a_4dvarnet_sla.png} \\
\vspace{-2mm}
%%%%% KINETIC ENERGY %%%%%%%%
\includegraphics[trim={0 0 42mm 0},clip, width=3.20cm,height=3cm]{content/figures/maps/ke/dc20a/nadir4/dc20a_nemo_ke.png} &
\includegraphics[trim={0 0 42mm 0},clip, width=3.2cm,height=3cm]{content/figures/maps/ke/dc20a/nadir4/dc20a_miost_ke.png} &
\includegraphics[trim={0 0 42mm 0},clip, width=3.2cm,height=3cm]{content/figures/maps/ke/dc20a/nadir4/dc20a_bfnqg_ke.png} &
\includegraphics[width=4.0cm,height=3cm]{content/figures/maps/ke/dc20a/nadir4/dc20a_4dvarnet_ke.png}  \\
\vspace{-2mm}
%%%%% RELATIVE VORTICITY %%%%%%%%
\includegraphics[trim={0 0 42mm 0},clip, width=3.20cm,height=3cm]{content/figures/maps/rvort/dc20a/nadir4/dc20a_nemo_vort_r.png} &
\includegraphics[trim={0 0 42mm 0},clip, width=3.2cm,height=3cm]{content/figures/maps/rvort/dc20a/nadir4/dc20a_miost_vort_r.png} &
\includegraphics[trim={0 0 42mm 0},clip, width=3.2cm,height=3cm]{content/figures/maps/rvort/dc20a/nadir4/dc20a_bfnqg_vort_r.png} &
\includegraphics[width=4.0cm,height=3cm]{content/figures/maps/rvort/dc20a/nadir4/dc20a_4dvarnet_vort_r.png}  \\
%%%%% STRAIN %%%%%%%%
\includegraphics[trim={0 0 38mm 0},clip, width=3.20cm,height=3cm]{content/figures/maps/strain/dc20a/nadir4/dc20a_nemo_strain.png} &
\includegraphics[trim={0 0 38mm 0},clip, width=3.2cm,height=3cm]{content/figures/maps/strain/dc20a/nadir4/dc20a_miost_strain.png} &
\includegraphics[trim={0 0 38mm 0},clip, width=3.2cm,height=3cm]{content/figures/maps/strain/dc20a/nadir4/dc20a_bfnqg_strain.png} &
\includegraphics[width=4.0cm,height=3cm]{content/figures/maps/strain/dc20a/nadir4/dc20a_4dvarnet_strain.png}  \\
% \vspace{-2mm}
(a) & (b) & (c) & (d)
\end{tabular}
\vspace{-3mm}
% \caption{Row I - Isotrophic PSD. Row 2 - Isotrophic PSD Score}
\caption{
A snapshot at $27^{th}$ October, 2012 of the sea level anomaly (SLA) from the NEMO simulation for the OSSE experiment outlined in section~\ref{sec:experimental_design}. 
The top row showcases the aggregated NADIR altimetry tracks and the aggregated SWOT altimetry tracks (12 hours before and 12 hours after) as well as the SST from the NEMO simulation.
Each subsequent row showcases the following physical variables found in appendix~\ref{sec:physical_variables}: (a) Sea Level Anomaly, (b) Kinetic Energy, (c) Relative Vorticity, and (d) Strain. 
Each column in the subsequent rows showcase the following reconstructed field from the NEMO simulation found in columrn (a): (b) MIOST~\cite{MIOST}, (c) BFN-QG~\cite{BFNQG}, and (d) 4DVarNet~\cite{4DVARNETSWOT}.}
\vspace{-5mm}
\label{fig:oceanbench_maps}
\end{center}
\end{figure}


% \subsubsection{Observing System Experiments (OSE)} \label{sec:ose}

\textbf{Observing System Experiments (OSE)}. As more observations have become available over the past few decades, we can also design experiments using real data. 
This involves aggregating as many observations from real ocean altimetry satellites as possible with some specific independent subset left out for evaluation purposes.
A major downside to OSE experiments is that the sparsity and spatial coverage of the observations narrow the possible scope of performance metrics and make it very challenging to learn directly from observation datasets. 
The current standard altimetry data are high resolution but cover a tiny area. 
As such, it can only inform fine-scale SSH patterns in the along-track satellite direction and cannot explicitly reveal two-dimensional patterns. 
Despite these drawbacks, it provides a quantitative evaluation of the generalizability of the ML methods concerning the true ocean state.
%and so it fails to capture many of the dynamical regimes we are interested in, i.e. mesoscale and sub-mesoscale processes. 
%However, it is still advantageous (and preferable) to include these experiments because these reflect the true ocean state and will help with the generalizability of the ML methods.

\begin{figure}[t!]
\small
\begin{center}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ccc}
% $\mathcal X$ & $\hat \z = \bG_\theta(\x)$ & $\x = \bG_\theta^{-1} (\hat \z)$\\[0mm]
% NATL60&
% \multicolumn{2}{c}{\includegraphics[width=6.25cm,height=4.5cm]{content/figures/exp_natl60/psd_st/osse_2020a_psd_natl60}} 
% \\
\includegraphics[width=3.75cm,height=3.25cm]{content/figures/stats/nrmse_space.png} &
\includegraphics[width=4.25cm,height=3.5cm]{content/figures/psd_isotropic/dc20a/nadir4/dc20a_psd_iso_ssh.png} &
\includegraphics[width=4.25cm,height=3.5cm]{content/figures/psd_isotropic/dc20a/nadir4/dc20a_psd_score_iso_ssh.png} 
\\
(a) Normalized RMSE &
(b) Isotropic Power Spectrum &
(c) Isotropic Power Spectrum Score
\end{tabular}
\begin{tabular}{cccc}
\includegraphics[trim={0 0 0mm 0},clip, width=4.20cm,height=3cm]{content/figures/psd_spacetime/dc20a/nadir4/dc20a_psd_spacetime_nemo_nadir4_ssh.png}  &
\includegraphics[trim={20mm 0 34mm 0},clip, width=2.9cm,height=3cm]{content/figures/psd_spacetime/dc20a/nadir4/dc20a_psd_spacetime_score_miost_nadir4_ssh.png} &
\includegraphics[trim={20mm 0 34mm 0},clip, width=2.9cm,height=3cm]{content/figures/psd_spacetime/dc20a/nadir4/dc20a_psd_spacetime_score_bfnqg_nadir4_ssh.png} &
\includegraphics[trim={20mm 0 0 0},clip, width=3.5cm,height=3cm]{content/figures/psd_spacetime/dc20a/nadir4/dc20a_psd_spacetime_score_4dvarnet_nadir4_ssh.png} \\
(d) NEMO Simulation &
(e) MIOST &
(f) BFN-QG &
(g) 4DVarNet
\end{tabular}
% % \vspace{-4mm}
% \caption{Row I - Isotrophic PSD. Row 2 - Isotrophic PSD Score}
\caption{This figure showcases some statistics for evaluation of the SSH field reconstructions for the OSSE NADIR experiment outlined in section~\ref{sec:interp_challenge}. Subfigure (a) showcases the normalized root mean squared error (nRMSE), (b) showcases the isotropic power spectrum decomposition (PSD), (c) showcases isotropic PSD scores.
The bottom row showcases the space-time PSD for the NEMO simulation (subfigure (d)) and the PSD scores for three reconstruction models: (e) the MIOST model~\cite{MIOST}, (f) the BFN-QG model~\cite{BFNQG}, and (g) the 4DVarNet model~\cite{4DVARNETSWOT}.
}
% \vspace{-5mm}
\label{fig:oceanbench_psd}
\end{center}
\end{figure}


%
\subsection{Data Challenges} \label{sec:data_challenges}



We rely on existing OSSE and OSE experiments for SSH interpolation designed by domain experts~\cite{DCOSEGULFSSH,DCOSSEGULFSSH} and recast them into \texttt{OceanBench} framework to deliver a ML-ready benchmarking suites. 
The selected data challenges  for this first edition address SSH interpolation for a 1000km$\times$1000km Gulfstream region. We briefly outline them below.
%The \textit{Ocean-Data-Challenge} group has a wide-range of different OSSE and OSE experiments involving SSH interpolation in particular~\cite{DCOSEGULFSSH,DCOSSEGULFSSH}. 
%For this paper, we will focus on a subset and demonstrate some evaluation steps generated from the \texttt{OceanBench} framework.
%We outline an experimental setup SSH reconstruction over the Gulfstream with three OSSE's configurations and one OSE configuration in the next section. For more detailed information about the experimental setups for each configuration, see section~\ref{sec:data_challenges_extended} in the appendix.

% \begin{itemize}
%     \item 
\textbf{Experiment I (\textit{OSSE NADIR})} addresses SSH interpolation using NADIR altimetry tracks which are very fine, thin ocean satellite observations (see Figure~\ref{fig:oceanbench_maps}). It relies on an OSSE using high-resolution ($1/60^\circ$ resolution) ocean simulations generated by the NEMO model over one year with a whole field every day. 

%The observation data uses NADIR altimetry tracks which are very fine, thin ocean satellite observations (see Figure~\ref{fig:oceanbench_maps} (a) \& (b)). 
\textbf{Experiment II (\textit{OSSE SWOT})} addresses SSH interpolation using jointly NADIR and SWOT altimetry data where we complement the \textbf{OSSE NADIR} configuration with simulated SWOT observations.
SWOT is a new satellite altimetry mission with a much higher spatial coverage but a much lower temporal resolution as illustrated in Figure~\ref{fig:oceanbench_maps}.
The higher spatial resolution allows us to see structures at a smaller resolution but at the cost of a massive influx of observations (over $\times$100).

\textbf{Experiment III (\textit{OSSE SST})} addresses SSH interpolation using altimetry and SST satellite data jointly. We complement the \textbf{OSSE SWOT} challenge with simulated SST observations. 
Satellite-derived SST observations are more abundantly available in natural operational settings than SSH at a finer resolution, and structures have visible similarities~\cite{SWOT,BFNQG}.
So this challenge allows for methods to take advantage of multi-modal learning~\cite{4DVARNETSST,SSHInterpAttention}.

\textbf{Experiment IV (\textit{OSE NADIR})} addresses SSH interpolation for real NADIR altimetry data. 
In contrast to the three OSSE data challenges, it only looks at actual observations aggregated from the currently available ocean altimetry data from actual satellites. 
It involves a similar space-time sampling as Experiment (\textbf{OSSE NADIR}) to evaluate the generalization of ML methods trained in Experiment I to real altimetry data. 
The training problem's complexity increases significantly due to the reference dataset's sparsity compared with the \textbf{OSSE NADIR} dataset. 
One may also explore transfer learning or fine-tuning strategies from the available OSSE dataset. 


% \begin{itemize}
%     \item Experiment I (\textbf{OSSE NADIR}) addresses SSH interpolation using NADIR altimetry tracks which are very fine, thin ocean satellite observations (see Figure~\ref{fig:oceanbench_maps}). It relies on an OSSE using anocean simulations generated by the NEMO model, more precisely a high-resolution simulation, $1/60^\circ$ resolution, over one year with a whole field every day. 
% %The observation data uses NADIR altimetry tracks which are very fine, thin ocean satellite observations (see Figure~\ref{fig:oceanbench_maps} (a) \& (b)). 
% \item Experiment II (\textbf{OSSE SWOT}) addresses SSH interpolation using jointly NADIR and SWOT altimetry data. We complement the \textbf{OSSE NADIR} configuration with simulated SWOT observations.  
% SWOT is a new satellite altimetry mission with  much higher spatial coverage but a much lower temporal resolution as illustrated in Figure~\ref{fig:oceanbench_maps}.
% The higher spatial resolution allows us to see structures at a smaller resolution but at the cost of a massive influx of observations (over $\times 100$).
% \item Experiment III (\textbf{OSSE SST}) addresses SSH interpolation using 
% jointly altimetry and SST satellite data. We complement the \textbf{OSSE SWOT} challenge with simulated SST observations. 
% Satellite-derived SST observations are more abundantly available in natural operational settings than SSH at a finer resolution, and structures have visible similarities \cite{}.
% So this challenge allows for methods to take advantage of multi-modal learning \cite{}.
% \item Experiment IV \textbf{OSE NADIR} addresses SSH interpolation for real NADIR altimetry data. In contrast to the three OSSE data challenges, it only looks at actual observations aggregated from the currently available ocean altimetry data from actual satellites. It involves a similar space-time sampling as Experiment (\textbf{OSSE NADIR}) to evaluate the generalization of ML methods trained in Experiment I to real altimetry data. Besides, one may also explore learning or fine-tuning strategies from the available OSE dataset. We may point out that the complexity of the training problem due to the sparsity of refence dataset compared with \textbf{OSSE NADIR} dataset.
% \end{itemize}




\subsection{\texttt{OceanBench} Pipelines}

\begin{table}[h]
\caption{This table highlights some of the results for the \textbf{OSSE NADIR} experiment outlined in section~\ref{sec:data_challenges} and appendix~\ref{sec:data_challenges_extended}.
% and the OSE experiment outlined in section~\ref{sec:ose}~\tocite{}. 
% For more results regarding the SWOT data, please see section~\ref{sec:other_tasks}. 
This table highlights the performance statistically in the real and spectral space; the normalized RMSE score for the real space and the minimum spatial and temporal scales resolved in the spectral domain. 
For more information about the class of models displayed and class of metrics, see appendix~\ref{sec:ml_ontology} and appendix~\ref{sec:metrics} respectively. We only showcase the model performance on the alongtrack NADIR data available. For the extended table for each of the challenges, see Table~\ref{tb:exp-results-mega}.}
\label{tb:oceanbench_results}
\centering
\begin{tabular}{lllcccc}
 \toprule
% Experiment & Configuration & Method & nRMSE & Resolved Scale [km]    \\ \midrule
% \multirow{2}{*}{Experiment} & \multirow{2}{*}{Algorithm} & \multirow{2}{*}{Algorithm Class} & \multirow{2}{*}{nRMSE} & \multicolumn{2}{c}{Effective Resolution} \\ 
% &  &   &  & Wavelength [km]  & Period [days]      \\ \midrule
% \multirow{2}{*}{Experiment} & \multirow{2}{*}{Algorithm} & \multirow{2}{*}{Algorithm Class} & \multirow{2}{*}{nRMSE} & \multicolumn{2}{c}{Effective Resolution} \\ 
Experiment &  Algorithm &   Algorithm Class &  nRMSE Score & $\lambda_{\mathbf{x}}$ [km]  & $\lambda_{t}$ [days]      \\ \midrule
\multicolumn{1}{l}{OSSE NADIR}     &  OI~\cite{DUACS} &  Coordinate-Based & 0.92 $\pm$ 0.01 & 175 & 10.8 \\
\multicolumn{1}{l}{OSSE NADIR}     &  MIOST~\cite{MIOST} &  Coordinate-Based  & 0.93 $\pm$ 0.01 & 157 & 10.1 \\
\multicolumn{1}{l}{OSSE NADIR}     &  BFNQG~\cite{BFNQG} &  Hybrid Model   & 0.93 $\pm$ 0.01 & 139 & 10.6 \\
OSSE NADIR &  4DVarNet~\cite{4DVARNETSWOT} &  Bi-Level Opt.  & 0.95 $\pm$ 0.01 & 117 & 7.7 \\
\bottomrule
\end{tabular}
\end{table}



For the four data challenges presented in the previous section, we used \texttt{OceanBench} pipelines to deliver a ML-ready benchmarking framework.
We used the \texttt{hydra} and the geoprocessing tools outlined in section~\ref{sec:code_structure} with specialized routines for regridding the ocean satellite data to a uniformly gridded product and vice versa when necessary. 
Appendix~\ref{sec:hydra_recipes} showcases an example of the hydra integration for the preprocessing pipeline. 
A key feature is the creation of a custom patcher for the appropriate geophysical variables using our \texttt{XRPatcher} tool, which is later integrated into custom datasets and dataloaders for the appropriate model architecture, e.g., coordinate-based or grid-based. 
We provide an example snippet of how this can be done easily in section~\ref{sec:xrpatcher}.
\texttt{OceanBench} also features some tools specific to the analysis of SSH. 
For example, physically-interpretable variables like geostrophic currents and relative vorticity, which can be derived from first-order and second-order derivatives of the SSH, are essential for assessing the quality of the reconstructions generated by the models. 
Figure~\ref{fig:oceanbench_maps} showcases some fields of the most common physical variables used in the oceanography literature for the SSH-based analysis of sea surface dynamics. For more details regarding the nature of the physical variables, see appendix~\ref{sec:physical_variables}.



Regarding the evaluation framework, we include domain-relevant performance metrics beyond the standard ML loss and accuracy functions. They account for the sampling patterns of the evaluation data. Spectral analytics are widely used in geoscience~\cite{BFNQG}, and here, we consider spectral scores computed as the minimum spatial and temporal scales resolved by the reconstruction methods proposed in~\cite{BFNQG}.
For example, figure~\ref{fig:oceanbench_psd} showcases how \texttt{OceanBench} generated the isotropic power spectrum and score and the space-time power spectrum decomposition and score.
Table~\ref{tb:oceanbench_results} outlines some standard and domain-specific scores for the experiments outlined in section~\ref{sec:experimental_design}.
We give a more detailed description of the rationale and construction of the power-spectrum-specific metrics in appendix~\ref{sec:metrics}. In terms of baselines, we report for each data challenge the performance of at least one approach for each of the category outlined in Section \ref{sec:ml_ontology_mini}.


% \begin{table}[h]
% \caption{This table highlights some of the results for the \textbf{OSSE NADIR} experiment outlined in section~\ref{sec:data_challenges} and appendix~\ref{sec:data_challenges_extended}.
% % and the OSE experiment outlined in section~\ref{sec:ose}~\tocite{}. 
% % For more results regarding the SWOT data, please see section~\ref{sec:other_tasks}. 
% This table highlights the performance statistically in the real and spectral space; the normalized RMSE for the real space and the minimum spatial and temporal scales resolved in the spectral domain. 
% For more information about the class of models displayed and class of metrics, see appendix~\ref{sec:ml_ontology} and appendix~\ref{sec:metrics} respectively. We only showcase the model performance on the alongtrack NADIR data available. For the extended table for each of the challenges, see Table~\ref{tb:exp-results-mega}.}
% \label{tb:oceanbench_results}
% \centering
% \begin{tabular}{lllcccc}
%  \toprule
% % Experiment & Configuration & Method & nRMSE & Resolved Scale [km]    \\ \midrule
% % \multirow{2}{*}{Experiment} & \multirow{2}{*}{Algorithm} & \multirow{2}{*}{Algorithm Class} & \multirow{2}{*}{nRMSE} & \multicolumn{2}{c}{Effective Resolution} \\ 
% % &  &   &  & Wavelength [km]  & Period [days]      \\ \midrule
% % \multirow{2}{*}{Experiment} & \multirow{2}{*}{Algorithm} & \multirow{2}{*}{Algorithm Class} & \multirow{2}{*}{nRMSE} & \multicolumn{2}{c}{Effective Resolution} \\ 
% Experiment &  Algorithm &   Algorithm Class &  nRMSE & $\lambda_{\mathbf{x}}$ [km]  & $\lambda_{t}$ [days]      \\ \midrule
% \multicolumn{1}{l}{OSSE NADIR}     &  OI (app.~\ref{sec:oi}) &  Coordinate-Based & 0.91 $\pm$ 0.01 & 176 & 11.6\\
% \multicolumn{1}{l}{OSSE NADIR}     &  MIOST~\ &  Coordinate-Based  & 0.92 $\pm$ 0.01 & 157 & 10.3 \\
% % \multicolumn{1}{l}{OSSE Gulf}     &  NerF &  Coordinate-Based  & 0.92 $\pm$ 0.01 & ... &\\
% \multicolumn{1}{l}{OSSE NADIR}     &  BFNQG (app.~\ref{sec:bfn}) &  Hybrid Model   & 0.92 $\pm$ 0.01 & 139 & 10.6 \\
% OSSE NADIR &  4DVarNet (app.~\ref{sec:4dvarnet}) &  Bi-Level Opt.  & 0.95 $\pm$ 0.01 & 117 & 7.7 \\
% % \bottomrule
% % OSE Gulf     &  OI &  Coordinate-Based  & ... & ... &\\
% % \multicolumn{1}{l}{OSE Gulf}     &  MIOST &  Coordinate-Based  & ... & ... &\\
% % \multicolumn{1}{l}{OSE Gulf}     &  NerF &  Coordinate-Based  & ... & ... &\\
% % \multicolumn{1}{l}{OSE Gulf}     &  BFNQG &  Hybrid Model  & ... & ... &\\
% % \multicolumn{1}{l}{OSE Gulf}     &  4DVarNet &  Bi-Level Opt.  & ... & ... &\\
% \bottomrule
% \end{tabular}
% \end{table}



==> content/5_conclusions.tex <==
\section{Conclusions} \label{sec:conclusions}

The ocean community faces technological and algorithmic challenges to make the most of available observation and simulation datasets. 
In this context, recent studies evidence the critical role of ML schemes in reaching breakthroughs in our ability to monitor ocean dynamics for various space-time scales and processes. 
Nevertheless, domain-specific preprocessing steps and evaluation procedures slow down the uptake of ML toward real-world applications. 
Our application of choice was SSH mapping which facilities the production of many crucial derived products that are used in many downstream tasks like subsequent modeling~\citep{ML4OCN}, ocean health monitoring~\citep{ML4NATURECONSERVATION,OCNHEALTH,OCEANHEALTH2} and maritime risk assessment~\citep{SSHOPERATIONAL}.

Through \texttt{OceanBench} framework, we embed domain-level requirements into the MLOPs considerations by building a flexible framework that adds this into the hyperparameter considerations for ML models. 
We proposed four challenges towards a ML-ready benchmarking suite for ocean observation challenges. 
We outlined the inner workings \texttt{OceanBench} and demonstrated its usefulness by recreating some preprocessing and analysis pipelines from a few data challenges involving SSH interpolation.
We firmly believe that the \texttt{OceanBench} platform is a crucial step to lowering the barrier of entry for new ML researchers interested in applying and developing their methods to relevant problems in the ocean sciences.





==> content/a1_usecase_tools.tex <==
\section{Example Use: Shared ToolKit}

\subsection{Geoprocessing}


\subsection{Evaluation}

==> content/custom.tex <==
\newcommand\YAMLcolonstyle{\color{red}\mdseries}
\newcommand\YAMLkeystyle{\color{black}\bfseries}
\newcommand\YAMLvaluestyle{\color{blue}\mdseries}

\makeatletter

% here is a macro expanding to the name of the language
% (handy if you decide to change it further down the road)
\newcommand\language@yaml{yaml}

\expandafter\expandafter\expandafter\lstdefinelanguage
\expandafter{\language@yaml}
{
  keywords={true,false,null,y,n},
  keywordstyle=\color{darkgray}\bfseries,
  basicstyle=\YAMLkeystyle,                                 % assuming a key comes first
  sensitive=false,
  comment=[l]{\#},
  morecomment=[s]{/*}{*/},
  commentstyle=\color{purple}\ttfamily,
  stringstyle=\YAMLvaluestyle\ttfamily,
  moredelim=[l][\color{orange}]{\&},
  moredelim=[l][\color{magenta}]{*},
  moredelim=**[il][\YAMLcolonstyle{:}\YAMLvaluestyle]{:},   % switch to value style at :
  morestring=[b]',
  morestring=[b]",
  literate =    {---}{{\ProcessThreeDashes}}3
                {>}{{\textcolor{red}\textgreater}}1     
                {|}{{\textcolor{red}\textbar}}1 
                {\ -\ }{{\mdseries\ -\ }}3,
}

% switch to key style at EOL
\lst@AddToHook{EveryLine}{\ifx\lst@language\language@yaml\YAMLkeystyle\fi}
\makeatother

\newcommand\ProcessThreeDashes{\llap{\color{cyan}\mdseries-{-}-}}


\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{pythonstyle}{
    % backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=pythonstyle}

==> content/d_datasets.tex <==
\subsection{Datasets} \label{sec:datasets}

\subsubsection{GulfStream OSSE}

\begin{figure}[t!]
\small
\begin{center}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ccc}
% $\mathcal X$ & $\hat \z = \bG_\theta(\x)$ & $\x = \bG_\theta^{-1} (\hat \z)$\\[0mm]
% NATL60&
% \multicolumn{2}{c}{\includegraphics[width=6.25cm,height=4.5cm]{content/figures/exp_natl60/psd_st/osse_2020a_psd_natl60}} 
% \\
\includegraphics[width=4.25cm,height=3cm]{content/figures/maps/ssh/dc20a_nemo_ssh.png} &
\includegraphics[width=4.25cm,height=3cm]{content/figures/maps/ssh/dc20a_nadir4_ssh.png} 
&
\includegraphics[width=4.25cm,height=3cm]{content/figures/maps/ssh/dc20a_swot1_ssh.png} 
% &
% \includegraphics[width=6.25cm,height=4.5cm]{content/figures/maps/sla/dc20a_ssh_anomaly_nadir4_2012-10-27.png} 
\\
(a) NEMO Simulation & (b) NADIR Tracks &
(c) SWOT Tracks
\end{tabular}
% % \vspace{-4mm}
% \caption{Row I - Isotrophic PSD. Row 2 - Isotrophic PSD Score}
\caption{A snapshot at $27^{th}$ October, 2012 of the sea surface height (SSH) from the NEMO simulation for the OSSE experiment outlined in section~\ref{sec:data_challenges}. (a) showcases the full surface field and (b) showcases the aggregated alongtrack observations from the altimeters (12 hours before and 12 hours after).}
\vspace{-5mm}
\label{fig:maps}
\end{center}
\end{figure}

\subsubsection{GulfStream OSE}

\subsubsection{Mediterrenean OSE}

\subsubsection{GulfStream OSE}

==> content/demo.tex <==
\begin{lstlisting}[language=yaml]
---
key: value
map:
    key1: "foo:bar"
    key2: value2
list:
  - element1
  - element2
# This is a comment
listOfMaps:
  - key1: value1a
    key2: value1b
  - key1: value2a
    key2: value2b
---
\end{lstlisting}

\begin{lstlisting}[frame=single]
some
other
listing
\end{lstlisting}

\begin{minted}{yaml}
---
key: value
map:
    key1: "foo:bar"
    key2: value2
list:
  - element1
  - element2
# This is a comment
listOfMaps:
  - key1: value1a
    key2: value1b
  - key1: value2a
    key2: value2b
---
\end{minted}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PYTHON
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{minted}{python}
import numpy as np
    
def incmatrix(genl1,genl2):
    m = len(genl1)
    n = len(genl2)
    M = None #to become the incidence matrix
    VT = np.zeros((n*m,1), int)  #dummy variable
    
    #compute the bitwise xor matrix
    M1 = bitxormatrix(genl1)
    M2 = np.triu(bitxormatrix(genl2),1) 

    for i in range(m-1):
        for j in range(i+1, m):
            [r,c] = np.where(M2 == M1[i,j])
            for k in range(len(r)):
                VT[(i)*n + r[k]] = 1;
                VT[(i)*n + c[k]] = 1;
                VT[(j)*n + r[k]] = 1;
                VT[(j)*n + c[k]] = 1;
                
                if M is None:
                    M = np.copy(VT)
                else:
                    M = np.concatenate((M, VT), 1)
                
                VT = np.zeros((n*m,1), int)
    
    return M
\end{minted}


==> content/g_userstories.tex <==
\section{Target Audience}
% \subsection{Project Vision}
While this tool is general in scope, we specifically target three audiences: 1) the domain expert who may want to use and understand and investigate SSH in relation to other important EO quantities, 2) machine learning researchers who may want to investigate how to make a better model for SSH interpolation, and 3) downstream users who are interested in adopting some techniques for their own domain-specific applications that may rely on SSH like tracking ocean currents~\tocite{}, investigating biogeochemical transport~\tocite{}, or global climate change~\tocite{}. In the following subsections, we give a more detailed description about the users and how might they benefit from \texttt{OceanBench}.

\textbf{Domain Experts}. We consider \textit{domain experts} who are experts in different domains of oceanography. ...


\textbf{ML Researchers}. We consider those who are expert ML researchers but may lack...



\textbf{Down Stream Users}. We also envision a broader adoption of the framework across research labs interested in having standardized data challenges for their own research purposes. There are independent groups choosing datasets for their specific use cases however, this framework can serve as an easy way to integrate their existing methodologies into the set of common tools to be used and improved by multiple communities. By establishing a relatively consistent problem set, we hope that any innovation can be easily understood and transferred across domains.

==> content/neurips_template.tex <==
\section{Submissions to the NeurIPS 2023 Track on Datasets and Benchmarks}

Please read the instructions below carefully and follow them faithfully.

\subsection{Style}

Papers must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.

Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.

\subsection{Retrieval of style files}

The style files for the NeurIPS Track on Datasets and Benchmarks and other information are available on the World Wide Web at
\begin{center}
  \url{http://www.neurips.cc/Conferences/2023/CallForDatasetsBenchmarks}
\end{center}
The file \verb+neurips_data_2023.pdf+ contains these instructions and illustrates the
various formatting requirements your submission must satisfy.

The only supported style file for NeurIPS 2023 is \verb+neurips_data_2023.sty+,
written for \LaTeXe{}. There are no supported style sheets for Microsoft Word, RTF, or other formats. The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.

\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to the NeurIPS Track on Datasets and Benchmarks.

At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies. Note that submissions to the NeurIPS Track on Datasets and Benchmarks are reviewed in a single-blind fashion and therefore not anonymous. This is because datasets can typically not be shared in a non-anonymous way. If you feel strongly that your work should be submitted anonymously, please use the \verb+anonymous+ option. This will create a version of your work with all author names hidden.

The file \verb+neurips_data_021.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.

The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.

The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.

Authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.

Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

All headings should be lower case (except for first word and proper nouns),
flush left, and bold.

First-level headings should be in 12-point type.

\subsection{Headings: second level}

Second-level headings should be in 10-point type.

\subsubsection{Headings: third level}

Third-level headings should be in 10-point type.

\paragraph{Paragraphs}

There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone.

\subsection{Citations within the text}

The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.

The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}

If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2023+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}

If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2023}
\end{verbatim}

As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''

\subsection{Footnotes}

Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).

Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}

\subsection{Figures}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.

You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PDF files}

Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''

Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.

\begin{itemize}

\item You should directly generate PDF files using \verb+pdflatex+.

\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.

\item The IEEE has recommendations for generating PDF files whose fonts are also
  acceptable for NeurIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.

\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.

\end{itemize}

If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.

\subsection{Margins in \LaTeX{}}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})

A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

\subsection{Suppressing line numbers in supplementary materials}
If you need to suppress line numbers in the supplementary materials because 
they interfere with the text, for instance because you are including a 
data sheet in 2-column format, you can do so by
placing the following command before it:
\begin{verbatim}
    \let\linenumbers\nolinenumbers\nolinenumbers
\end{verbatim}
